Spectral properties of Type Ia supernovae up to z~0.3

Aims: Spectroscopic observations of Type Ia supernovae obtained at the New Technology Telescope (NTT) and the Nordic Optical Telescope (NOT), in conjunction with the SDSS-II Supernova Survey, are analysed. We use spectral indicators measured up to a month after the lightcurve peak luminosity to characterise the supernova properties, and examine these for potential correlations with host galaxy type, lightcurve shape, colour excess, and redshift. Methods: Our analysis is based on 89 Type Ia supernovae at a redshift interval z = 0.05 - 0.3, for which multiband SDSS photometry is available. A lower-z spectroscopy reference sample was used for comparisons over cosmic time. We present measurements of time series of pseudo equivalent widths and line velocities of the main spectral features in Type Ia supernovae. Results: Supernovae with shallower features are found predominantly among the intrinsically brighter slow declining supernovae. We detect the strongest correlation between lightcurve stretch and the Si ii 4000 absorption feature, which also correlates with the estimated mass and star formation rate of the host galaxy. We also report a tentative correlation between colour excess and spectral properties. If confirmed, this would suggest that moderate reddening of Type Ia supernovae is dominated by effects in the explosion or its immediate environment, as opposed to extinction by interstellar dust.

==> nttnotspec.tex <==
\longtab{2}{
\begin{longtable}{p{1.0cm}p{1.0cm}p{3cm}p{3cm}}
\caption{\label{tab:sdsspec} NTT/NOT spectra.} \\
\hline \hline
ID & IAU & SPID & Epochs (days) \\
\hline
\endfirsthead
\caption{continued.}\\
\hline\hline
ID & IAU SPID & Epochs (days) \\
\hline
\endhead
\hline
\endfoot
\endlastfoot
12781&2006er&680&10.9\\
12843&2006fa&727&10.2\\
12853&2006ey&685&10.3\\
12856&2006fl&695&-3.2\\
12860&2006fc&688&-1.9\\
12898&2006fw&712&-6.6\\
12930&2006ex&687&10.1\\
12950&2006fy&700&-4.4\\
13025&2006fx&761&3.4\\
13044&2006fm&724, 1062&-8.2, 20.2\\
13070&2006fu&736&6.9\\
13072&2006fi&723&0.0\\
13135&2006fz&739, 998&-7.7, 17.6\\
13796&2006hl&1058, 1058&12.7, 12.7\\
13894&2006jh&1039&9.2\\
14157&2006kj&1040&9.4\\
14437&2006hy&1061&14.0\\
14846&2006jn&1014&-1.7\\
14871&2006jq&1008&-4.2\\
14979&2006jr&1009&-2.1\\
14984&2006js&1027&-1.2\\
15129&2006kq&1015&1.8\\
15132&2006jt&1012&-2.4\\
15161&2006jw&1010&-1.0\\
15171&2006kb&1045, 1045&-5.7, -5.7\\
15203&2006jy&1026&-2.4\\
15222&2006jz&1004&-5.8\\
15259&2006kc&1051&-1.9\\
16021&2006nc&1355&11.3\\
16069&2006nd&1467&11.5\\
16165&2006nw&1326&2.6\\
16215&2006ne&1456&4.3\\
16287&2006np&1449, 1449, 1569, 1569, 1650&2.4, 2.4, 3.3, 3.3, 19.5\\
16352&2006pk&1478&4.1\\
16473&2006pl&1520&1.3\\
16637&&1514&-0.9\\
17332&2007jk&1899&3.3\\
17366&2007hz&1782&8.9\\
17389&2007ih&1811&7.0\\
17435&2007ka&1902, 1902&2.7, 2.7\\
17497&2007jt&1837&-2.4\\
17552&2007jl&1789&3.5\\
17745&2007ju&2161&15.1\\
17784&2007jg&1842&-5.5\\
17790&2007jx&1887&1.0\\
17811&2007ix&1816, 1816&4.6, 4.6\\
17825&2007je&1819&-4.9\\
17875&2007jz&1817&0.3\\
17880&2007jd&1843, 1957&-1.9, 1.2\\
17886&2007jh&1844&-4.5\\
18325&2007mv&2277&8.6\\
18466&2007lm&2270&4.5\\
18768&2007lh&2135&6.7\\
18787&2007mf&2150&0.2\\
18804&2007me&2148&-5.0\\
19023&2007ls&2236&-1.7\\
19101&2007ml&2268, 2268&-6.0, -6.0\\
19149&2007ni&2275, 2275&-7.1, -7.1\\
19155&2007mn&2607&18.7\\
19282&2007mk&2280&-8.2\\
19341&2007nf&2298&-2.4\\
19353&2007nj&2281&-7.3\\
19381&2007nk&2283, 2283&-3.5, -3.5\\
19899&2007pu&2550&1.2\\
19913&2007qf&2585&9.6\\
19953&2007pf&2602&4.2\\
19968&2007ol&2549&5.2\\
20039&2007qh&2584&7.6\\
20040&2007rf&2612&6.4\\
20142&2007qg&2586&4.7\\
20144&2007ql&2541&1.1\\
20345&2007qp&2567, 2567&-0.7, -0.7\\
20364&2007qo&2581&-1.3\\
20430&2007qj&2543&1.4\\
20625&2007px&2551, 2604&-5.4, -3.6\\
21006&2007qs&2566&1.7\\
21033&2007qy&2565&-3.3\\
21034&2007qa&2719&13.3\\
21042&2007qz&2564&-6.4\\
21422&2007rq&2599&-3.6\\
21502&2007ra&2574, 2575&-8.6, -7.7\\
\end{longtable}
}


==> snspectra.tex <==
\longtab{1}{
\begin{longtable}{p{1.2cm}p{4cm}p{4cm}p{4cm}}
\caption{\label{tab:snspectra} Supernova spectra.} \\
\hline \hline
SN & epochs (days) & Spec source & LC source\\
\hline
\endfirsthead
\caption{continued.}\\
\hline\hline
SN & epochs (days) & Spec source & LC source\\
\hline
\endhead
\hline
\endfoot
\endlastfoot
SN1983g & 6, 7 & \citet{1992AA...259...63C} & - \\
SN1986g & -4, -4, -4, -3, -3, -2, -1, 0, 1, 21 & \citet{2002AJ....124..417H} & \citet{2008AA...492..535A} \\
SN1989b & 0, 6, 11, 21, 22 & \citet{1990AA...237...79B} & \citet{2008AA...492..535A} \\
SN1990n & 2 & \citet{1993AA...269..423M,1998AJ....115.1096G} & \citet{2008AA...492..535A} \\
SN1991bg & 1, 1, 2, 2, 16, 18, 20, 29 & \citet{1996MNRAS.283....1T,1996AJ....112.2094G} & \citet{2008AA...492..535A} \\
SN1991m & 3, 28 & \citet{1998AJ....115.1096G} & \citet{2008AA...492..535A} \\
SN1991s & 14 & \citet{1998AJ....115.1096G} & - \\
SN1991t & -12, -11, -10, -9, -8, -7, -6 & \citet{1995AA...297..509M,1998AJ....115.1096G} & \citet{2008AA...492..535A} \\
SN1992g & 15 & \citet{1998AJ....115.1096G} & - \\
SN1994d & -11, -11, -10, -9, -8, -5, -4, -2, 2, 2, 3, 4, 4, 5, 7, 10, 10, 11, 11, 12, 13, 15, 17, 19, 24, 26 & \citet{1996MNRAS.278..111P,1998AJ....115.1096G} & \citet{2008AA...492..535A} \\
SN1994q & 10 & \citet{1996AJ....112.2094G} & - \\
SN1994s & 22 & \citet{1996AJ....112.2094G} & \citet{2009ApJ...700.1097H} \\
SN1996x & -4, -2, -1, 0, 1, 3, 7, 12, 22, 24 & \citet{2001MNRAS.321..254S} & \citet{2008ApJ...686..749K} \\
SN1997br & -9, -8, -7, -6, -4, 8, 24 & \citet{1999AJ....117.2709L} & \citet{2008AA...492..535A} \\
SN1997cn & 3, 28 & \citet{1998AJ....116.2431T} & \citet{2008AA...492..535A} \\
SN1997do & -12, -11, -8, -7, 8, 10, 11, 12, 14, 15, 20, 21 & \citet{2008AJ....135.1598M} & \citet{2008ApJ...686..749K} \\
SN1997dt & -11, -10, -9, -8, -5, 0, 2 & \citet{2008AJ....135.1598M} & \citet{2008ApJ...686..749K} \\
SN1998ab & -8, 17, 18, 19, 20, 21, 22 & \citet{2008AJ....135.1598M} & \citet{2009ApJ...700.1097H} \\
SN1998aq & -9, -8, -3, 0, 0, 1, 1, 2, 2, 3, 3, 4, 4, 5, 5, 6, 6, 7, 18, 19, 20, 21, 23, 24, 30 & \citet{2008AJ....135.1598M,2003AJ....126.1489B} & \citet{2008AA...492..535A} \\
SN1998bu & -4, -4, -3, -3, -2, -2, 0, 8, 8, 9, 9, 10, 10, 10, 11, 11, 12, 12, 13, 13, 27, 27, 28, 28, 29, 29, 30 & \citet{2008AJ....135.1598M,1999IAUC.7149....2J,2001ApJ...549L.215C,2004AA...426..547S} & \citet{2008AA...492..535A} \\
SN1998dh & -9, -9, -8, -6, -4, -1 & \citet{2008AJ....135.1598M} & \citet{2008ApJ...686..749K} \\
SN1998dm & 4, 5, 7, 10, 12, 15, 17, 24 & \citet{2008AJ....135.1598M} &  \\
SN1998eg & -1, 4, 5, 17, 19, 23 & \citet{2008AJ....135.1598M} & \citet{2009ApJ...700.1097H} \\
SN1998v & 0, 1, 2, 11, 12, 14 & \citet{2008AJ....135.1598M} & \citet{2009ApJ...700.1097H} \\
SN1999aa & -11, -11, -10, -9, -8, -7, -7, -7, -6, -5, -4, -3, -3, -3, -2, -1, -1, 0, 5, 5, 6, 6, 14, 14, 14, 15, 16, 17, 19, 19, 25, 25, 27, 28, 28, 28, 29, 30 & \citet{2008AJ....135.1598M,2004AJ....128..387G,2007AA...470..411G} & \citet{2009ApJ...700.1097H} \\
SN1999ac & -15, -15, -11, -9, -9, -3, 0, 0, 2, 2, 2, 7, 8, 8, 11, 11, 16, 16, 24, 28, 28 & \citet{2008AJ....135.1598M,2005AJ....130.2278G,2006AJ....131.2615P,2007AA...470..411G} & \citet{2008ApJ...686..749K} \\
SN1999af & -5, 1, 15, 17, 17, 25 & \citet{2007AA...470..411G} & - \\
SN1999ao & 5, 7, 9, 12, 17 & \citet{2007AA...470..411G} & \citet{2009ApJ...700.1097H} \\
SN1999ar & 5 & \citet{2007AA...470..411G} & \citet{2009ApJ...700.1097H} \\
SN1999au & 11, 15, 18, 21 & \citet{2007AA...470..411G} & - \\
SN1999av & 2, 5, 9, 30 & \citet{2007AA...470..411G} & - \\
SN1999aw & 3, 5, 9, 12, 15, 23, 30 & \citet{2007AA...470..411G} & \citet{2009ApJ...700.1097H} \\
SN1999be & 14, 19, 26 & \citet{2007AA...470..411G} & - \\
SN1999bi & 5, 11, 12, 26 & \citet{2007AA...470..411G} & \citet{2009ApJ...700.1097H} \\
SN1999bk & 4, 6, 8 & \citet{2007AA...470..411G} & - \\
SN1999bm & 3, 5, 24 & \citet{2007AA...470..411G} & \citet{2009ApJ...700.1097H} \\
SN1999bn & 2, 12, 19, 24 & \citet{2007AA...470..411G} & \citet{2009ApJ...700.1097H} \\
SN1999bp & -2, 0, 1, 6, 16, 21 & \citet{2007AA...470..411G} & \citet{2009ApJ...700.1097H} \\
SN1999bq & 3, 3, 16, 20, 24 & \citet{2007AA...470..411G} & - \\
SN1999by & -5, -5, -4, -4, -3, -3, -2, -2, 1, 2, 3, 3, 3, 4, 4, 5, 5, 6, 6, 6, 7, 7, 8, 9, 10, 11, 16, 24, 25, 28, 29 & \citet{2008AJ....135.1598M,2004ApJ...613.1120G,2007AA...470..411G} & \citet{2008AA...492..535A} \\
SN1999cc & -4, -2, -1, 1, 18, 23, 25 & \citet{2008AJ....135.1598M} & \citet{2009ApJ...700.1097H} \\
SN1999ee & -11, -9, -4, -2, 0, 5, 7, 9, 14, 17, 20, 25, 30 & \citet{2002AJ....124..417H} & \citet{2008AA...492..535A} \\
SN1999ej & -1, 2, 4, 8, 11 & \citet{2008AJ....135.1598M} & \citet{2008ApJ...686..749K} \\
SN1999gd & 2, 9, 27 & \citet{2008AJ....135.1598M} & \citet{2009ApJ...700.1097H} \\
SN1999gp & -5, -2, 0, 3, 5, 7, 22 & \citet{2008AJ....135.1598M} & \citet{2009ApJ...700.1097H} \\
SN2000cf & 3, 4, 14, 16, 24, 25 & \citet{2008AJ....135.1598M} & \citet{2009ApJ...700.1097H} \\
SN2000cn & -10, -9, -8, 8, 10, 12, 21, 26, 27 & \citet{2008AJ....135.1598M} & \citet{2009ApJ...700.1097H} \\
SN2000cx & -4, -3, -2, -1, 0, 1, 5, 6, 7, 9, 11, 14, 19, 22, 24, 26, 28, 30 & \citet{2008AJ....135.1598M,2001PASP..113.1178L} & \citet{2008AA...492..535A} \\
SN2000dk & -5, -4, 1, 4, 9 & \citet{2008AJ....135.1598M} & \citet{2009ApJ...700.1097H} \\
SN2000e & -9, -6, -5, 5 & \citet{2003ApJ...595..779V} & \citet{2008AA...492..535A} \\
SN2000fa & -11, -11, 1, 2, 4, 9, 11, 14, 16, 18, 20 & \citet{2008AJ....135.1598M} & \citet{2009ApJ...700.1097H} \\
SN2001el & 9, 14, 22 & \citet{2003ApJ...591.1110W} & \citet{2003AJ....125..166K} \\
SN2001v & -14, -13, -12, -11, -10, -8, -7, -6, -4, 9, 10, 11, 12, 13, 18, 19, 20, 20, 21, 21, 22, 23, 24, 27, 28 & \citet{2008AJ....135.1598M,2008AJ....135.1598M} & \citet{2003AA...397..115V} \\
SN2002bo & -14, -13, -11, -6, -5, -5, -4, -3, -3, -2, -1, 4, 28 & \citet{2004MNRAS.348..261B} & \citet{2008AA...492..535A} \\
SN2002dj & -11, -10, -9, -8, -6, -4, -3, 9, 10, 13, 17, 22 & \citet{2008MNRAS.388..971P} & \citet{2009ApJ...700.1097H} \\
SN2002er & -11, -9, -8, -7, -6, -5, -4, -3, -2, -1, 0, 2, 4, 5, 6, 10, 12, 13, 16, 17, 20, 25 & \citet{2005AA...436.1021K} & \citet{2008AA...492..535A} \\
SN2003cg & -9, -8, -7, -5, -2, -2, -1, 1, 4, 7, 10, 11, 12, 16, 19, 23, 23, 26, 28 & \citet{2006MNRAS.369.1880E} & \citet{2008AA...492..535A} \\
SN2003du & -13, -11, -11, -11, -8, -7, -6, -5, -4, -3, -2, -1, 0, 0, 1, 2, 2, 3, 4, 6, 6, 7, 8, 9, 9, 10, 13, 15, 17, 18, 19, 21, 24, 26 & \citet{2007AA...469..645S,2005AA...429..667A,2005ASPC..342..250G} & \citet{2008AA...492..535A} \\
SN2004dt & -10, -9, -9, -7, -7, -6, -6, -4, -4, -3, -2, -1, -1, 2, 3, 4, 14, 17, 21 & \citet{2007AA...475..585A} & - \\
SN2004eo & -11, -6, -3, 2, 7, 11, 13, 14, 21, 22, 24, 30 & \citet{2007MNRAS.377.1531P} & \citet{2008AA...492..535A} \\
SN2004s & 1, 7, 12, 13, 13, 18 & \citet{2007AJ....133...58K} & \citet{2008AA...492..535A} \\
SN2005bl & -6, -5, -3, -3, 4, 12, 19, 21 & \citet{2008MNRAS.385...75T} & - \\
SN2005cf & -12, -12, -11, -10, -10, -9, -7, -7, -6, -4, -3, -1, 0, 4, 4, 5, 6, 7, 9, 12, 12, 14, 16, 25, 29 & \citet{2007AA...471..527G,2007AIPC..937..311L} & \citet{2008AA...492..535A} \\
SN2005cg & -10, -9, -4, 0, 5, 7 & \citet{2006ApJ...636..400Q} & - \\
SN2005hj & -6, 0, 2, 5 & \citet{2007ApJ...666.1083Q} & \citet{2009ApJ...700.1097H} \\
SN2005hk & -8, -7, -6, -6, -5, -4, -4, -3, 4, 13, 15, 24, 27 & \citet{2007PASP..119..360P} & \citet{2008AA...492..535A} \\
SN2006gz & -14, -14, -13, -13, -12, -10, -9, -5, -2, 5, 6, 7, 8, 8, 9, 10, 11 & \citet{2007ApJ...669L..17H} & \citet{2008AA...492..535A} \\
SN2006x & -10, -7, 0 & \citet{2009PASJ...61..713Y} & - \\
\end{longtable}
}

